Interpretable Acoustic Representation Learning on Breathing and Speech Signals for COVID-19 Detection

In this paper, we describe an approach for representation learning of audio signals for the task of COVID-19 detection. The raw audio samples are processed with a bank of 1-D convolutional filters that are parameterized as cosine modulated Gaussian functions. The choice of these kernels allows the interpretation of the filterbanks as smooth band-pass filters. The filtered outputs are pooled, log-compressed and used in a self-attention based relevance weighting mechanism. The relevance weighting emphasizes the key regions of the time-frequency decomposition that are important for the downstream task. The subsequent layers of the model consist of a recurrent architecture and the models are trained for a COVID-19 detection task. In our experiments on the Coswara data set, we show that the proposed model achieves significant performance improvements over the baseline system as well as other representation learning approaches. Further, the approach proposed is shown to be uniformly applicable for speech and breathing signals and for transfer learning from a larger data set.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> figs/fig_relev_boxplot.tex <==
\begin{figure*}[t!]
    \centering
    %\includegraphics[width=0.8\textwidth, trim = 30mm 0mm 38mm 0mm, clip]{LaTeX/figs/clsRelWt_boxPlot_wt_dist-crop.pdf}
    \includegraphics[width=0.8\textwidth]{figs/clsRelWt_boxPlot_wt_dist-crop.pdf}
    \caption{Variation of relevance weights across frequency bands for COVID-19 positive (pos) and negative(neg) classes.} 
    \label{fig:relev_box}
\end{figure*}

==> figs/fig_relevance_weights.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=.45\textwidth]{figs/br_preTr_relWt_dist_xbands-crop.pdf}
    \caption{Variation of average acoustic relevance weights across frequency for COVID-19 positive and negative classes.} 
    \label{fig:relevance}
\end{figure}

==> tables/res_breathing.tex <==
\begin{table}[tb]
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|cccccc}
\hline
% \small
\footnotesize{Representation} & \multicolumn{1}{l}{\footnotesize{Fold1}} & \multicolumn{1}{l}{\footnotesize{Fold2}} & \multicolumn{1}{l}{\footnotesize{Fold3}} & \multicolumn{1}{l}{\footnotesize{Fold4}} & \multicolumn{1}{l}{\footnotesize{Fold5}} & \multicolumn{1}{l}{\footnotesize{Avg.}} \\ \hline
\footnotesize{Mel-Spectrogram} & \footnotesize{73.8} & \footnotesize{76.4} & \footnotesize{75.6} & \footnotesize{77.1} & \footnotesize{84.2} & \footnotesize{77.4} \\
\footnotesize{SincNet} & \footnotesize{72.4} & \footnotesize{69.6} & \footnotesize{81.9} & \footnotesize{76.4} & \footnotesize{77.1} & \footnotesize{75.4} \\
\hdashline[1pt/1pt]
\footnotesize{CosGaus-rel} & \footnotesize{75.4} & \footnotesize{76.0} & \footnotesize{79.7} & \footnotesize{78.1} & \footnotesize{82.8} & \footnotesize{78.4} \\
\footnotesize{CosGaus-rel-modFB} &  \footnotesize{72.2} & \footnotesize{70.4} &  \footnotesize{79.4} &  \footnotesize{76.7} & \footnotesize{81.9} & \footnotesize{76.1}  \\
\footnotesize{CosGaus-rel-modFB-rel} & \footnotesize{73.7} & \footnotesize{76.0} & \footnotesize{81.1} & \footnotesize{78.3} & \footnotesize{82.9} & \footnotesize{78.4} \\
%Cos-Gauss-relev-pretr. & 76.1 & 75.9 & 77.7 & 76.9 & 83.2 & 78.0 \\
\footnotesize{CosGaus-rel-pretr-fine} & \footnotesize{\textbf{81.2}} & \footnotesize{\textbf{77.0}} & \footnotesize{\textbf{80.9}} & \footnotesize{\textbf{78.4}} & \footnotesize{\textbf{84.9}} & \textbf{\footnotesize{80.5}} \\ \hline
\end{tabular}
\caption{Comparison of different representations on breathing modality in terms of the AUC.}
\end{table}

==> tables/res_cough.tex <==
\begin{table}[H]
\begin{tabular}{lcccccc}
\hline
Representation & \multicolumn{1}{l}{fold1} & \multicolumn{1}{l}{fold2} & \multicolumn{1}{l}{fold3} & \multicolumn{1}{l}{fold4} & \multicolumn{1}{l}{fold5} & \multicolumn{1}{l}{Avg.} \\ \hline
Mel & 71.5 & 79.7 & 78.3 & 74.8 & 73.9 & 75.6 \\
SincNet & {\color[HTML]{1A1A1A} 63.1} & {\color[HTML]{1A1A1A} 69.8} & {\color[HTML]{1A1A1A} 63.0} & {\color[HTML]{1A1A1A} 66.1} & {\color[HTML]{1A1A1A} 70.2} & {\color[HTML]{1A1A1A} 66.4} \\
Cos-Gauss-relev & 72.3 & 79.2 & 76.1 & 78.9 & 80.8 & \textbf{77.4} \\
SincNet-relev-pretr-fine & {\color[HTML]{1A1A1A} 68.1} & {\color[HTML]{1A1A1A} 62.5} & {\color[HTML]{1A1A1A} 67.0} & {\color[HTML]{1A1A1A} 72.7} & {\color[HTML]{1A1A1A} 69.0} & {\color[HTML]{1A1A1A} 67.9} \\
Cos-Gauss-relev-pretr-fine & 74.8 & 74.8 & 76.0 & 66.1 & 82.7 & 74.9 \\ \hline
\end{tabular}
\caption{Comparison of different representations on cough}
\end{table}

==> tables/res_speech.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|cccccc}
\hline
% \small
\footnotesize{Representation} & \multicolumn{1}{l}{\footnotesize{Fold1}} & \multicolumn{1}{l}{\footnotesize{Fold2}} & \multicolumn{1}{l}{\footnotesize{Fold3}} & \multicolumn{1}{l}{\footnotesize{Fold4}} & \multicolumn{1}{l}{\footnotesize{Fold5}} & \multicolumn{1}{l}{\footnotesize{Avg.}} \\ \hline
\footnotesize{Mel-Spectrogram} & \footnotesize{74.8} & \footnotesize{85.1} & \footnotesize{79.1} & \footnotesize{78.6} & \footnotesize{80.4} & \footnotesize{79.6} \\
\footnotesize{SincNet} & \footnotesize{ }  & \footnotesize{ } & \footnotesize{ } & \footnotesize{ } & \footnotesize{ } & \footnotesize{ }\\
\hdashline[1pt/1pt]
\footnotesize{CosGaus-rel} & \footnotesize{76.5} & \footnotesize{83.6} & \footnotesize{83.3} & \footnotesize{79.6} & \footnotesize{84.5} & \footnotesize{81.5} \\
\footnotesize{CosGaus-rel-modFB} & \footnotesize{ } & \footnotesize{ } & \footnotesize{ } & \footnotesize{ } & \footnotesize{ } & \footnotesize{ } \\
\footnotesize{CosGaus-rel-modFB-rel} & \footnotesize{75.6} & \footnotesize{79.4} & \footnotesize{80.7} & \footnotesize{81.2} & \footnotesize{82.6} & \footnotesize{79.9}\\
%Cos-Gauss-relev-pretr. &  & &  &  &  &  \\
\footnotesize{CosGaus-rel-pretr-fine} & \footnotesize{78.3} & \footnotesize{81.5} & \footnotesize{83.5} & \footnotesize{78.0} & \footnotesize{81.5} & \footnotesize{80.6} \\ \hline
\end{tabular}
\caption{Comparison of different representations on speech modality in terms of the AUC.}
\end{table}
